Social Media Analysis for Crisis Informatics in the Cloud

Social media analysis of disaster events is a critical task in crisis informatics research. It involves analyzing social media data generated during natural disasters, crisis events, or other mass convergence events. Due to the large data sets generated during these events, large scale software infrastructures need to be designed to analyze the data in a timely manner. Creating such infrastructures bring the need to maintain them and this becomes more difficult as these infrastructures grow larger and older. Maintenance costs are high since there is a need for queries to be handled quickly which require large amounts of computational resources to be available on demand 24 hours a day, seven days a week. In this thesis, I describe an alternative approach to designing a software infrastructure for analyzing unstructured data on the cloud while providing fast queries and with the reliability needed for crisis informatics research. Additionally, I discuss a new approach for a more reliable Twitter stream collection using container orchestrated systems. I finally compare this new infrastructure with existing crisis informatics software infrastructures and compare their reliability, scalability and extensibility with my approach and my prototype.

==> chapter1.tex <==
\chapter{Introduction}
\label{introchap}

This sample document illustrates how to use the
{\tt thesis} class, originally written by John P. Weiss.
Some requirements of the Graduate School are written
into that file; page size, line spacing, appropriate
placement of captions for tables and figures, etc.
Revisions by Hongcheng Ni make it possible to use the
(optional)
\verb2\usepackage{hyperref}2 command to enable
internal hyperlinks in the final PDF document.
Other tasks of conforming to the requirements are
left to other existing \LaTeX{} packages.
For example, a common problem is to insert graphics ---
figures and tables --- into the body of the thesis.  For
this one should use the {\tt graphicx} package, which is
part of the standard \TeX{} distribution.  Likewise, the
Grad School specs say that a large table may be displayed
in landscape mode at reduced size, but its caption must
also be in rotated position, in the same font and size as
the normal text in the body of the thesis.  To accomplish
this, the user must invoke the {\tt rotating} package,
available online.


Figure \ref{xfigDiagram} shows an image from a PDF file
imported into this document
using the \verb2graphicx2 package.
The command \verb2\usepackage{graphicx}2, which appears
near the very top of the main \LaTeX{} file, reads in
this package which defines the
\verb2\includegraphics{}2 macro.


\begin{figure}[htbp]
	\caption[Cylinder and measurements]{
	This diagram of a cylinder and various
	measurements and quantities was actually
	made using {\bf xfig}, a freeware
	drawing program for Unix systems.
	Diagrams can be exported directly to PDF
	files, the preferred format for
	vector graphics.  Vector graphics can
	be magnified indefinitely without degradation,
	whereas bitmap images (JPG and PNG)
	must be pretty high-resolution if you don't
	want them looking all pixellated when
	magnified.
	}
    \begin{center}
	\includegraphics[width=100mm]{figs/cyl.pdf}
    \end{center}
\label{xfigDiagram}
\end{figure}


\begin{figure}[htbp]
    \caption[Bitmap images]{
	The JPEG bitmap format is great for photos but
	crummy for diagrams (including drawings, graphs,
	charts) because it can't gracefully handle sharp edges.
	Note the same bitmap image below from a PNG file and
	from a JPG file; the latter shows characteristic
	``ringing'' at sharp edges -- including text!
	Seriously, magnify and look closely at the JPG's
	awful lines and edges.
	Vector-format PDF is the best for diagrams, but
	if you must use a bitmap image, let it be PNG.
	~ (Left: file {\it drawing.png}.
	Right: file {\it drawing.jpg}.)
	}
    \begin{center}
	\includegraphics[width=70mm]{figs/drawing.png}
	${}^{}$ ~
	${}^{}$ ~
	${}^{}$
	\includegraphics[width=70mm]{figs/drawing.jpg}
    \end{center}
\label{bitmapImages}
\end{figure}



\section{Lists in {\tt thesis} class}

In {\tt thesis} class (for Colorado University),
lists are defined so that nested lists will be
numbered or marked appropriately.
First, an itemized (non-enumerated) list
prefaces each item with a bullet.
Nested itemized list use asterisks,
then dashes, then dots.
These lists are typed between
the \verb2\begin{itemize}2
and \verb2\end{itemize}2
commands.

\begin{itemize}
  \item{} This is ``itemized'' item A.
  \item{} This is ``itemized'' item B.
  \item{} This is ``itemized'' item C.
  \begin{itemize}
    \item{} This is ``itemized'' subitem A.
    \begin{itemize}
      \item{} This is ``itemized'' subsubitem A.
      \begin{itemize}
        \item{} This is ``itemized'' subsubsubitem A.
      \end{itemize}
      \item{} This is ``itemized'' subsubitem B.
    \end{itemize}
    \item{} This is ``itemized'' subitem B.
  \end{itemize}
  \item{} This is ``itemized'' item D.
\end{itemize}

Enumerated lists use the commands
\verb2\begin{enumerate}2 and
\verb2\end{enumerate}2,
and nested enumerations appear like this.

\begin{enumerate}
  \item{} This is ``enumerated'' item A.
  \item{} This is ``enumerated'' item B.
  \item{} This is ``enumerated'' item C.
  \begin{enumerate}
    \item{} This is ``enumerated'' subitem A.
    \begin{enumerate}
      \item{} This is ``enumerated'' subsubitem A.
      \begin{enumerate}
        \item{} This is ``enumerated'' subsubsubitem A.
      \end{enumerate}
      \item{} This is ``enumerated'' subsubitem B.
    \end{enumerate}
    \item{} This is ``enumerated'' subitem B.
  \end{enumerate}
  \item{} This is ``enumerated'' item D.
\end{enumerate}


The work presented
here\footnote{Footnotes are handled neatly by \LaTeX.}
is an extension of Lao\cite{lao:thesis}
and Lao et~al.\cite{lao:paper},
fictional references that are in the bibliographic
source file \verb9refs.bib9.

\begin{table}[htb]
    \caption[Example of a table with its own footnotes]{
	Here is an example of a table with its own footnotes.
	Don't use the $\backslash${\tt footnote} macro if you
	don't want the footnotes at the bottom of the page.
	Also, note that in a thesis the caption goes
	\emph{above} a table, unlike figures.
	}
    \begin{center}
    \begin{tabular}{||l|c|c|c|c||} \hline
	& $S$ & $P$ &   $Q^{\ast}$  & $D^{\dagger}$ \\	% footnote symbols!
	wave form & (kVA) & (kW) & (kVAr) & (kVAd) \\  \hline \hline
	Fig.  \ref{xfigDiagram}a  & 25.48 & 25.00 & -2.82 & 4.03 \\ \hline
	Fig.  \ref{xfigDiagram}b  & 25.11 & 18.02 & -9.75 & 14.52 \\ \hline
	Table \ref{pdftable}  & 24.98 & 22.26 & 9.19 & 6.64 \\ \hline
	Table \ref{powertable}  & 23.48 & 15.00 & 6.59 & 16.82 \\ \hline
	Fig.  \ref{pyramid}  & 24.64 & 22.81 & -0.44 & 9.3 \\ \hline
	\end{tabular}
   \\ \rule{0mm}{5mm}
   ${}^\ast$kVAr means reactive power.		% footnote symbol
\\ ${}^\dagger$kVAd means distortion power.	% footnote symbol
\end{center}
\label{powertable}
\end{table}




==> chapter2.tex <==
\chapter{Mathematical Formulation}
\label{mathchapter}

The objective of this fake thesis document is to demonstrate
a multitude of \LaTeX{} features as well as features specific
to the thesis class.
We start by giving one short formula,
and one big hairy multi-line formula
(one of the non-dimensional Navier-Stokes equations):

\begin{equation}
	A = \pi r^2
\end{equation}


\begin{eqnarray}
  \rho \left[ \frac{DV_r}{Dt} - M \epsilon^2
    \frac{\vth^2}{r} \right]
  & = & -\frac{\delta^2}{\gamma~ M} \diffr{P}
	+ \frac{M ~\delta^2}{Re} \left\{ 2 \diffr{}
	\left[ \mu \left( \diffr{V_r}
        - \frac{1}{3} {\bf \nabla \cdot \overline{V}}
      \right) \right] \right. \nonumber \\
  & & + \frac{1}{r} \diffth{} \left[ \mu \left(
      \frac{1}{r} \diffth{V_r} + \epsilon \diffr{\vth}
      - \epsilon \frac{\vth}{r} \right) \right] \nonumber \\
  & & + \diffz{} \left[ \mu \left( \frac{1}{\delta^2}
        \diffz{V_r} + \diffr{V_z} \right) \right] \nonumber \\
  & & + 2 \left. \frac{\mu}{r}\left[ \diffr{V_r} -\frac{\epsilon}{r}
      \diffth{\vth} - \frac{V_r}r\right] \right\}, \label{eq:rmom}
\end{eqnarray}


\section{Explanation of equations}

The latter equation is non-dimensionalized using the following definitions:

\[
	r = \frac{r'}{R'}, ~~~
	z = \frac{z'}{L'},~~~
	t = \frac{t'}{t_a'}, ~~~
	\kappa = \frac{\kappa'}{\kappa_0'}, ~~~
	\mu = \frac{\mu'}{\mu_0'} , ~~~
	C_V = \frac{C_V'}{C_{V0}'},
\]
where $P_0'$ is the initial static pressure in the cylinder,
and $\rho_0'$ and $T_0'$ are the density and temperature
of the fluid being injected from the sidewall.

\begin{figure}[htbp]
    \caption[Cutting up a triangular pyramid]{
	A triangular pyramid may be cut up as shown, to
	yield one top pyramid (with one-eighth the volume
	of the full pyramid), three bottom corner pyramids
	(which, when joined, are congruent to the top pyramid),
	three prisms along the bottom edges (the area of whose
	bottom faces total $B/2$) and the large central prism
	(volume = $(B/4)(h/2) = Bh/8$).
	The image, from PDF file ``pyr.pdf'',
	was read in using the {\tt $\backslash$includegraphics}
	command, from the {\tt graphicx} package.
	}
    \begin{center}
	\includegraphics[width=90mm]{figs/pyr.pdf}
    \end{center}
\label{pyramid}
\end{figure}


Here is an example of using the macros
\verb2\singlespacing2 and \verb2\doublespacing2:

\singlespacing	% <------------------------------

This paragraph was preceded by the
command \verb2\singlespacing2.
See the Specifications of the Grad School for instructions
about when single spacing is appropriate in a thesis.

\doublespacing	% <------------------------------

And now, here is an example of using the macros
\verb2\begin{singlespace}2 and \verb2\end{singlespace}2;
another way to get single-spacing.

\begin{singlespace}	% <-----------------------------
Two cases are studied in the present work which differ only in the
boundary conditions.  Each different boundary condition model a
different source of instability.  The boundary of the first case
consists of a steady, axisymmetric sidewall radial velocity boundary
and a time-dependent, non-axisymmetric endwall axial velocity
boundary.  The second case is studied with a fixed impermeable axial
velocity along the endwall and a combination axisymmetric steady and
non-axisymmetric unsteady radial velocity along the sidewall.
\end{singlespace}	% <-----------------------------


Usually you want to use a table produced by some other
software, such as Excel, rather than try to do it using
\LaTeX macros.  If the table is saved/printed to a PDF file,
then it can be displayed using the
$\backslash${\tt includegraphics} macro
inside a {\tt table} environment:


\begin{table}
    \caption[Table from a PDF file]{
	This table wasn't constructed with \LaTeX{}
	commands, but resides in PDF file
	({\tt tableD.pdf})
	created by some other software.
	}
    \begin{center}
	\includegraphics[width=5.45in]{figs/tableD.pdf}
    \end{center}
\label{pdftable}
\end{table}


Some of the boundary conditions are:

\begin{eqnarray}
  z=0; && V_z = \twochoices
	{0, && t\leq0}
	{\widetilde{F}_{zw}(r,\theta,t), && t>0}
						\label{eq:endwall} \\
  z=0; && V_{\theta}=V_r=0			\label{eq:endnoslip} \\
  r=0; && P,\rho,T,V_r,\vth,V_z~\mbox{finite},	\label{eq:centerline} \\
  r=1; && V_r= F_{rws}(z),			\label{eq:injection} \\
  r=1; && V_z=\vth =0,				\label{eq:sidenoslip}
\end{eqnarray}
and solutions must be periodic in $\theta$.

If you don't believe this stuff, check out
Mulick\cite{mulick} and Baylor\cite{baylor}.


\section{Yet another section}

\subsection{
	Just meaningless text to test lines per page
	\label{ss}}

According to the Grad School specs.   there should be 24--27 lines
of print per page of a thesis.  This should be true whether the font
size is 10, 11, or 12.  Count them up; does this document conform?
According to the Grad School specs.   there should be 24--27 lines
of print per page of a thesis.  This should be true whether the font
size is 10, 11, or 12.  Count them up; does this document conform?
According to the Grad School specs.   there should be 24--27 lines
of print per page of a thesis.  This should be true whether the font
size is 10, 11, or 12.  Count them up; does this document conform?
According to the Grad School specs.   there should be 24--27 lines
of print per page of a thesis.  This should be true whether the font
size is 10, 11, or 12.  Count them up; does this document conform?
According to the Grad School specs.   there should be 24--27 lines
of print per page of a thesis.  This should be true whether the font
size is 10, 11, or 12.  Count them up; does this document conform?
According to the Grad School specs.   there should be 24--27 lines
of print per page of a thesis.  This should be true whether the font
size is 10, 11, or 12.  Count them up; does this document conform?
According to the Grad School specs.   there should be 24--27 lines
of print per page of a thesis.  This should be true whether the font
size is 10, 11, or 12.  Count them up; does this document conform?
According to the Grad School specs.   there should be 24--27 lines
of print per page of a thesis.  This should be true whether the font
size is 10, 11, or 12.  Count them up; does this document conform?
According to the Grad School specs.   there should be 24--27 lines
of print per page of a thesis.  This should be true whether the font
size is 10, 11, or 12.  Count them up; does this document conform?
According to the Grad School specs.   there should be 24--27 lines
of print per page of a thesis.  This should be true whether the font
size is 10, 11, or 12.  Count them up; does this document conform?
According to the Grad School specs.   there should be 24--27 lines
of print per page of a thesis.  This should be true whether the font
size is 10, 11, or 12.  Count them up; does this document conform?
According to the Grad School specs.   there should be 24--27 lines
of print per page of a thesis.  This should be true whether the font
size is 10, 11, or 12.  Count them up; does this document conform?
According to the Grad School specs.   there should be 24--27 lines
of print per page of a thesis.  This should be true whether the font
size is 10, 11, or 12.  Count them up; does this document conform?
According to the Grad School specs.   there should be 24--27 lines
of print per page of a thesis.  This should be true whether the font
size is 10, 11, or 12.  Count them up; does this document conform?
According to the Grad School specs.   there should be 24--27 lines
of print per page of a thesis.  This should be true whether the font
size is 10, 11, or 12.  Count them up; does this document conform?
According to the Grad School specs.   there should be 24--27 lines
of print per page of a thesis.  This should be true whether the font
size is 10, 11, or 12.  Count them up; does this document conform?
According to the Grad School specs.   there should be 24--27 lines
of print per page of a thesis.  This should be true whether the font
size is 10, 11, or 12.  Count them up; does this document conform?

\paragraph{What is it?}
This is a labelled paragraph.
The heading of the paragraph is emphasized.
This is a labelled paragraph.
The heading of the paragraph is emphasized.

\subsection{This is a subsection}

This is a subsection.
Filler filler filler filler filler filler filler filler.
Filler filler filler filler filler filler filler filler.

\subsection{This is another subsection}

This is another subsection.
Filler filler filler filler filler filler filler filler.
Filler filler filler filler filler filler filler filler.

\paragraph{This is paragraph number 2.}
It used a \verb2\paragraph{}2 header, which
are always inlined (with extra space)
and  boldfaced.

This is the third paragraph of the subsection.
Filler filler filler filler filler filler filler filler.
Filler filler filler filler filler filler filler filler.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsubsection{This is a subsubsection (1)}
This is the first paragraph of the subsubsection.
Whether it is numbered or inlined depends on the
option selected at the beginning of the
thesis.

By default, a \verb2\subsubsection2 heading is numbered
and set off on a separate line, left-justified.

\paragraph{However.}
Using the \verb2inlineh42 option, subsubsection headers
are inlined.
And using the \verb2nonumh42 option suppresses
numbering of the subsubsections.
Together they make subsubsection headings
just the same as paragraph headings.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsubsection{
	This is another subsubsection (2)
	\label{sss}
	}

Once again, whether its heading is numbered
and/or inlined depends on the class options
chosen at the start.

There is no ``subsubsubsection'' entity,
and ``subparagraph'' gets no special treatment
in \emph{thesis} class.

\section{The End}
\label{sec:end}

Finally, this is the end.  The bibliography starts on
the next page.
Note how the \verb2\hyperref2 package
(mentioned in chapter \ref{introchap})
also makes hyperlinks from references
(e.g., Mulick\cite{mulick})
to entries in the bibliography.


